Efficiently Predicting Mutational Effect on Homologous Proteins by Evolution Encoding

Predicting protein properties is paramount for biological and medical advancements. Current protein engineering mutates on a typical protein, called the wild-type, to construct a family of homologous proteins and study their properties. Yet, existing methods easily neglect subtle mutations, failing to capture the effect on the protein properties. To this end, we propose EvolMPNN, Evolution-aware Message Passing Neural Network, an efficient model to learn evolution-aware protein embeddings. EvolMPNN samples sets of anchor proteins, computes evolutionary information by means of residues and employs a differentiable evolution-aware aggregation scheme over these sampled anchors. This way, EvolMPNN can efficiently utilise a novel message-passing method to capture the mutation effect on proteins with respect to the anchor proteins. Afterwards, the aggregated evolution-aware embeddings are integrated with sequence embeddings to generate final comprehensive protein embeddings. Our model shows up to 6.4% better than state-of-the-art methods and attains 36X inference speedup in comparison with large pre-trained models. Code and models are available at https://github.com/zhiqiangzhongddu/EvolMPNN.

==> pages/concept.tex <==
In many therapeutic areas, including oncology and genetic disease.
The ability to understand the structural impact of missense mutations can facilitate the design of therapeutics.
Over the last year or two, there have been differing views on the ability of AlphaFold2 to reliably model missense mutations.
\cite{BW22} compared AlphaFold2 structures with x-ray structures for three systems where x-ray structures for the wild-type protein were available, and specific structure-disrupting mutations existed.  
AlphaFold2 predicted similar structures for mutant and WT in all three cases and failed to recognise the structure-disrupting mutation~\cite{BW22}.
% 
This finding is consistent with~\cite{PMNPVMKI21}, which found that AlphaFold2 structures did not reproduce experimentally observed changes in protein stability or fluorescence associated with single mutations. 

However, all may not be lost.  
\cite{MBJWB22} provide promising evidence that RoseTTAFold can predict the structural impact of protein mutations. 

MSA algorithms are applied to families of evolutionarily related biological sequences (proteins, RNA or DNA) in order to infer sites in each sequence that are likely to be related
to one another, meaning that they descend from a common ancestor~\cite{WM21}. 
MSAs can be used as the basis for extrapolation:
for instance, knowledge about one region in one sequence
can be used to make guesses about related regions in related
sequences~\cite{WM21}. 
MSAs can also be used to understand biological
function: for instance, if particular amino acids at particular sites are highly conserved across sequences, it may be evidence that they are crucial to biological function~\cite{WM21}.

\textbf{What are multiple sequence alignment (MSA) and full MSA?}

\textbf{We can propose a benchmark for homologous protein understanding.}

\subsection{Remaining Challenges}
\begin{enumerate}
    \item It is unknown how far mutations' effect will propagate to their neighbours in physical and sequence space.
    \item The prediction model must be able to resolve the single-point mutation amid the length of protein sequence up to hundreds or even thousands of amino acids.
    \item It is not easy to find a complete MSA in practice. 
    Is MSA expensive? 
    \item 3D structure information estimation/prediction process is too slow to be feasible for millions of mutants. 
\end{enumerate}

\subsection{Research Goals}
\begin{enumerate}
    \item Accurate mutant property prediction.
    \item Efficient mutant property prediction.
    \begin{itemize}
        \item Giving an initial state can reduce the cost compared with completely training a model. 
    \end{itemize}
    \item Restrict the application case as datasets like AAV series?
    \begin{itemize}
        \item We focus on a specific application case.
        \item Different from other general models, MSA is very expensive in this case. 
        \item Predicting mutational effect on protein property of sequence families. 
        \item But in this case, rich MSA information will further boost the existing model's performance? 
        If yes, should we claim we are more efficient?
        \item Note that we don't have rich MSA information because MSA requires all sequences to have corresponding 3D structures.
    \end{itemize}
    \item Prediction of orphan and rapidly evolving proteins for which an MSA cannot be generated (or for which we have very shallow MSAs).
\end{enumerate}

\subsection{Research Contributions}
\begin{enumerate}
    \item Include graph structure in the model. 
    \begin{itemize}
        \item Mostly done. 
        We can obtain WT's 3D graph structure from AF2 as the initial structure of this sequence family.
        Then, we change the structure of each sequence during training. 
    \end{itemize}
    \item Avoid multiple sequence alignments (MSA). 
    \begin{itemize}
        \item It is probably impossible to avoid MSA if we want to capture evolutionary information.
        Unless we can find another way to identify sequence families from a massive protein database. 
        Do only AAV datasets have clear sequence families? 
    \end{itemize}
    \item Unsupervised and Supervised. 
\end{enumerate}

\subsection{TODO Tasks}
\begin{enumerate}
    \item \textbf{Research Goal.}
    \begin{enumerate}
        \item Our goal is to predict the 3D structure of mutants or predict the property of mutants.
        \begin{itemize}
            \item If we want to predict the 3D structure of mutants, is it a bit far from the AAVanguard project?
            \item If we want to predict the property of mutants, do we need to find more baselines?
        \end{itemize}
        \item We consider the influence of single mutation or simple mutations?
        \begin{itemize}
            \item If we only consider a single mutation, we can not use the evolution graph idea. 
            And it is not the setting of the AAVanguard project.
            \item If we consider simple mutations, \ie, $\geq 1$, do we need more baselines?
        \end{itemize}
    \end{enumerate}
    \item \textbf{Dataset.}
    \begin{enumerate}
        \item Do other datasets have mutants caused by different operations?
        \begin{itemize}
            \item AAV protein datasets have different operations. 
            \item Others? TODO
        \end{itemize}
    \end{enumerate}
    \item \textbf{Frameowrk Design.}
    \begin{enumerate}
        \item Evolution-based model.
        \begin{itemize}
            \item \cite{RMSGLLGOZM21,RLVMCASR21,MRVLSR21} utilise special design attention to capture evolutionary information from MSA. 
            Can we do it without MSA?
            \item Is MSA a good solution for homologous protein families?
        \end{itemize}
        \item 3D Structure-based model. 
        \begin{itemize}
            \item We can have 3D structure for WT.
        \end{itemize}
        \item Combined.
        \begin{itemize}
            \item TODO. 
        \end{itemize}
        \item How to construct protein graphs?
        \begin{itemize}
            \item Use AlphaFold2 to get graph structure for WTs and use WT's graph as the initial graph structure of related mutants. 
            \item The above solution still needs a Transformer structure - do we have better or novel solutions?
        \end{itemize}
        \item How to design specific parts for mutational information?
        \begin{itemize}
            \item TODO
        \end{itemize}
        \item How to represent evolutionary information?
        \begin{itemize}
            \item \textbf{Multiple sequence alignment (MSA):} MSA is a method to align homologous protein sequences and identify conserved regions, insertions, and deletions. 
            The MSA can be represented as a matrix or a sequence logo, where each position in the alignment shows the frequency of amino acids.
            \item \textbf{Phylogenetic tree:} A phylogenetic tree shows the evolutionary relationship between different members of a protein family. 
            The tree can be constructed based on the similarity of the sequences, using methods like maximum likelihood, Bayesian inference, or distance-based methods.
            \item \textbf{Protein structure:} Protein structures can reveal the functional and evolutionary constraints on a protein family. 
            Homology modeling, comparative modeling, or structural superposition can be used to compare the structures of different members of a protein family and identify conserved structural features.
            \item \textbf{Conserved domains and motifs:} Many protein families share conserved domains or motifs that are indicative of their evolutionary origin and function. 
            These can be identified using tools like Pfam, PROSITE, or InterPro.
            \item \textbf{Evolutionary rates and selection pressures:} 
            Evolutionary rates and selection pressures on different sites in a protein sequence can be estimated using methods like dN/dS ratio, which compares the rates of nonsynonymous and synonymous mutations.
        \end{itemize}
    \end{enumerate}
    \item \textbf{Experiments.}
\end{enumerate}

\subsection{Related Work}

\textbf{Facebook ESM.}
\begin{enumerate}
    \item MSA Transformer~\cite{RLVMCASR21}
    \begin{itemize}
        \item They combine Transformer with evolutionary information, i.e., using MSA and optimised attention. 
        \item Evaluate on structure prediction task. 
    \end{itemize}
    \item Biological Structure and Function Emerge from Scaling Unsupervised Learning to 250 Million Protein Sequences~\cite{RMSGLLGOZM21}
    \begin{itemize}
        \item ESM-1b model. 
        \item A protein Transformer trained on a large protein dataset. 
    \end{itemize}
    \item Language models enable zero-shot prediction of the effects of mutations on protein function~\cite{MRVLSR21}
    \begin{itemize}
        \item ESM-1v model. 
        \item For a given mutation, we can consider the amino acid in the wild-type protein as a reference state, comparing the probability assigned to the mutated amino acid with the probability assigned to the wild-type. 
    \end{itemize}
    \item Language models of protein sequences at the scale of evolution enable accurate structure prediction~\cite{LARHZLSFSCR22}
    \begin{itemize}
        \item ESM-2. 
        Its variants have up to 15 billion parameters, the largest language model of protein sequences to date
        \item ESMFold. 
        It uses the information and representations learned by ESM-2 to perform end-to-end 3D structure prediction using only a single sequence as input, allowing us to quantify the emergence of protein structure as the language model is scaled from millions to billions of parameters. 
        \item They train models up to 15 billion parameters, the largest language models of proteins to be evaluated to date. 
        \item Larger NLP model can capture important information which can be further used for folding. 
    \end{itemize}
    \item Evolutionary-scale prediction of atomic-level protein structure with a language model~\cite{LARHZLSVKS22}
    \begin{itemize}
        \item ESM-2. 
        \item ESMFold. 
        \item The first large-scale structural characterisation of metagenomic proteins. 
    \end{itemize}
\end{enumerate}

\textbf{DeepMind AlphaFold.}
\begin{enumerate}
    \item Highly accurate protein structure prediction with AlphaFold~\cite{JEPGFRTBZP21}
    \begin{itemize}
        \item AlphaFold2. 
    \end{itemize}
    \item Can AlphaFold2 predict the impact of missense mutations on structure?~\cite{BW22}
    \begin{itemize}
        \item They compared AlphaFold2 structures with x-ray structures for three systems where x-ray structures for the wild-type protein were available and specific structure-disrupting mutations existed.  
        \item AlphaFold2 predicted similar structures for mutant and WT in all three cases and failed to recognise the structure-disrupting mutation.
    \end{itemize}
    \item Using AlphaFold to predict the impact of single mutations on protein stability and function~\cite{PMNPVMKI21}
    \begin{itemize}
        \item They found that AlphaFold2 structures did not reproduce experimentally observed changes in protein stability or fluorescence associated with single mutations. 
    \end{itemize}
\end{enumerate}

\textbf{David Baker group RoseTTAFold.}
\begin{enumerate}
    \item Accurate prediction of protein structures and interactions using a three-track neural network~\cite{BDADOLWCKS21}
    \begin{itemize}
        \item RoseTTAFold.
    \end{itemize}
    \item Accurate Mutation Effect Prediction using RoseTTAFold~\cite{MBJWB22}
    \begin{itemize}
        \item They provide promising evidence that RoseTTAFold can predict the structural impact of protein mutations. 
        \item But they have not yet published their final version paper and their code. 
        Only reported some promising results. 
    \end{itemize}
\end{enumerate}

\textbf{Important related work}
\begin{enumerate}
    \item Structure-based protein function prediction using graph convolutional networks~\cite{GRKLBVCTFV21}
    \begin{itemize}
        \item They introduce DeepFRI, a GCN for predicting protein functions by leveraging sequence features extracted from a protein language model and protein structures.
        \item They use LSTM to capture sequence information.
        \item They apply GCN on a protein graph that is extracted from a protein contact map using 3D distance. 
    \end{itemize}
    \item Mutation effects predicted from sequence co-variation~\cite{HIPSSSM1717}
    \begin{itemize}
        \item They present EVmutation, an unsupervised statistical method for predicting the effects of mutations that explicitly captures residue dependencies between positions.
    \end{itemize}
    \item Deciphering interaction fingerprints from protein molecular surfaces using geometric deep learning~\cite{GSMRBBC20}
    \begin{itemize}
        \item TODO
    \end{itemize}
    \item Multi-Scale Representation Learning on Proteins~\cite{SBK21}
    \begin{itemize}
        \item This paper introduces a multi-scale graph construction of a protein – HOLOPROT – connecting surface to structure and sequence. 
        The surface captures coarser details of the protein, while sequence as primary component and structure – comprising secondary and tertiary components – capture finer details.
        \item The method is evaluated on two representative tasks, protein-ligand binding affinity and enzyme-catalysed reaction classification.
        \item MSMS~\cite{SOS96} \url{https://ssbio.readthedocs.io/en/latest/index.html}. 
    \end{itemize}
    \item PIVOTAL: prioritizing variants of uncertain significance with spatial genomic patterns in the 3D proteome~\cite{LMSCY21}
    \begin{itemize}
        \item They present a spatial neighbourhood-based method using three-dimensional structural models of proteins that significantly improves current variant prioritisation tools and identifies potential disease aetiology of candidate variants on a proteome scale. 
    \end{itemize}
    \item Predicting functional effect of missense variants using graph attention neural networks~\cite{ZXFCS22}
    \begin{itemize}
        \item Co-evolution captures the functional correlation between positions. 
        Recent studies~\cite{HIPSSSM1717,LMSCY21} have shown that co-evolution helps to improve prediction accuracy.
        \item They define star graphs where variants are centre nodes and connect with other 128 amino acids flanking the reference amino acid as protein context. 
    \end{itemize}
    \item Exploring evolution-aware \& -free protein language models as protein function predictors~\cite{HYYJSWYD22}
    \begin{itemize}
        \item It's also a MSA-based framework. 
    \end{itemize}
    \item Efficient evolution of human antibodies from general protein language models~\cite{HSXBWTWPK23}
    \begin{itemize}
        \item They report general protein language models can efficiently evolve human antibodies by suggesting mutations that are evolutionarily plausible, despite providing the model with no information about the target antigen, binding specificity or protein structure.
        \item However, I didn't see their technical contributions. 
    \end{itemize}
\end{enumerate}

\textbf{Other related work.}
\begin{enumerate}
    \item Correlated mutations and residue contacts in proteins~\cite{GSSV94}
    \begin{itemize}
        \item TODO
    \end{itemize}
    \item Identification of direct residue contacts in protein-protein interaction by message passing~\cite{WWSHH09}
    \begin{itemize}
        \item TODO
    \end{itemize}
    \item Improved contact prediction in proteins: Using pseudolikelihoods to infer Potts models~\cite{ELLWA13}
    \begin{itemize}
        \item An MSA identifies corresponding sites across a family of related sequences.
        \item TODO
    \end{itemize}
    \item Deep generative models of genetic variation capture the effects of mutations~\cite{RIM18}
    \begin{itemize}
        \item TODO
    \end{itemize}
    \item Learning inverse folding from millions of predicted structures~\cite{HVLLHSLR22}
    \begin{itemize}
        \item They study 3D structure to sequence problems. 
        The goal of inverse folding is to design sequences that fold to a desired structure.
    \end{itemize}
    \item Protein design and variant prediction using autoregressive generative models~\cite{SRKMSSMKM21}
    \begin{itemize}
        \item TODO
    \end{itemize}
    \item Best templates outperform homology models in predicting the impact of mutations on protein stability~\cite{PI22}
    \begin{itemize}
        \item TODO
    \end{itemize}
    \item Predicting single-point mutational effect on protein stability.
    \begin{itemize}
        \item A simple MLP incorporating only the embedding at the mutation site achieves a similar performance to the geometric model.
    \end{itemize}
    % \item Pre-training of Graph Neural Network for Modeling Effects of Mutations on Protein-Protein Binding Affinity~\cite{LLSP20}
    % \begin{itemize}
    %     \item TODO
    % \end{itemize}
    \item Transformer protein language models are unsupervised structure learners~\cite{RMSOR21}
    \begin{itemize}
        \item Transformer attention maps learn contacts from the unsupervised language modelling objective. 
    \end{itemize}
    \item Learning from Protein Structure with Geometric Vector Perceptrons~\cite{JESJTD21}
    \begin{itemize}
        \item They propose geometric vector perceptrons (GVPs), a drop-in replacement for standard multi-layer perceptrons (MLPs) in aggregation and feed-forward layers of GNNs.
        \item GVPs operate directly on both scalar and geometric features—features that transform as a vector under a rotation of spatial coordinates. 
        GVPs therefore allow for the embedding of geometric information at nodes and edges without reducing such information to scalars that may not fully capture complex geometry. 
    \end{itemize}
    \item Structure-aware Protein Self-supervised Learning~\cite{CZWLD22}
    \begin{itemize}
        \item TODO
    \end{itemize}
\end{enumerate}

There is a paper set about protein representation learning\footnote{\url{https://github.com/LirongWu/awesome-protein-representation-learning}}. 

\subsection{Dataset}

Some resources:
\begin{enumerate}
    \item Deep mutational scanning: A highly parallel method to measure the effects of mutation on protein function~\cite{SF15}
    \begin{itemize}
        \item TODO
    \end{itemize}
    \item ThermoMutDB: a thermodynamic database for missense mutations~\cite{XNKPRVAP21}
    \begin{itemize}
        \item TODO
    \end{itemize}
    \item Dissecting enzyme function with microfluidic-based deep mutational scanning~\cite{RTA15}
    \begin{itemize}
        \item They measure the susceptibility of beta-glucosidase (bgl3) to heat challenge in the dataset. 
    \end{itemize}
    \item Deep generative models of genetic variation capture the effects of mutations~\cite{RIM18} 
    \begin{itemize}
        \item TODO
    \end{itemize}
    \item FLIP: Benchmark tasks in fitness landscape inference for proteins~\cite{DMJWBGMY21}
    \begin{itemize}
        \item TODO
    \end{itemize}
    \item PEER: A Comprehensive and Multi-Task Benchmark for Protein Sequence Understanding~\cite{XZLZZMLT22}
    \begin{itemize}
        \item PEER is a comprehensive and multi-task benchmark for protein sequence understanding. 
        It contains 17 tasks of protein understanding lying in 5 task categories, including protein function prediction, protein localisation prediction, protein structure prediction, protein-protein interaction prediction and protein-ligand interaction prediction.
        \item It has the GB1 fitness prediction and AAV fitness prediction tasks, adopted from~\cite{DMJWBGMY21}.
        \item They provide some benchmark performances which can be used for our project. 
    \end{itemize}
    \item DeepLoc: prediction of protein subcellular localization using deep learning~\cite{ASSNW17}
    \begin{itemize}
        \item They work on a homologous protein dataset. 
        \item It is a dataset from DTU\footnote{\url{https://services.healthtech.dtu.dk/}}. 
    \end{itemize}
    \item A Differential Geometric View and Explainability of GNN on Evolving Graphs
    \item SimPer: Simple Self-Supervised Learning of Periodic Targets 
    \item 
    \item 
\end{enumerate}

\subsection{Baselines}
\begin{enumerate}
    \item Structure-based protein function prediction using graph convolutional networks~\cite{GRKLBVCTFV21}
    \item Predicting functional effect of missense variants using graph attention neural networks~\cite{ZXFCS22}
\end{enumerate}
